Make Prompt-based Black-Box Tuning Colorful: Boosting Model Generalization from Three Orthogonal Perspectives

Large language models (LLMs) have shown increasing power on various natural language processing (NLP) tasks. However, tuning these models for downstream tasks usually needs exorbitant costs or is unavailable due to commercial considerations. Recently, black-box tuning has been proposed to address this problem by optimizing task-specific prompts without accessing the gradients and hidden representations. However, most existing works have yet fully exploited the potential of gradient-free optimization under the scenario of few-shot learning. In this paper, we describe BBT-RGB, a suite of straightforward and complementary techniques for enhancing the efficiency and performance of black-box optimization. Specifically, our method includes three plug-and-play components: (1) Two-stage derivative-free optimization strategy that facilitates fast convergence and mitigates overfitting; (2) Automatic verbalizer construction with its novel usage under few-shot settings; (3) Better prompt initialization policy based on instruction search and auto-selected demonstration. Extensive experiments across various tasks on natural language understanding and inference demonstrate the effectiveness of our method. Our codes are publicly available at https://github.com/QiushiSun/BBT-RGB.

==> xnjbvwytkznyvkjxpkjxwdqtrytncvmf/algs/two-stage.tex <==
\begin{algorithm}[htb]
	\caption{Two-Stage DFOs (Detailed)}
	\label{alg:two-stage-detailed}
	\begin{algorithmic}[1]
		\Require \
		 popsize: $\lambda$, intrinsic dimension: $d$
            \Require \
          budget1:$b1$, budget2:$b2$, backbone:$f_{model}$
            \Require \
		 $m$, $\delta$, $C$, $D$  
     // initialize state variables
		\Ensure \
		hidden variable: $z$
		\Function{Two-Stage DFO}{}   
            \Statex\ // CMA-ES
            \Repeat
            \For{each hidden layer}
            \For{$i$ in 1 to $\lambda$}
            \State Sample $z_i$ from $\mathcal{N}$($m$,$\delta^2C$) 
            \State $f_i=f_{model}(z_i)$
            \EndFor
            \State Update $m, \delta, C$ with $f$
            \EndFor
            \State Update $z$ to min(f)
            \Until{ $b1$ times $f_{model}$ call}
            \Statex\ // COBYLA
            \For{each hidden layer}
            \Repeat
            \For{each search direction i in D}
            \State Update $z$ to min(f) along i
            \EndFor
            \State Select a new set of D
            \Until{ $b2//d$ times $f_{model}$ call}
            
            \EndFor
            % \EndFor
	    \EndFunction
	\end{algorithmic}
\end{algorithm}

==> xnjbvwytkznyvkjxpkjxwdqtrytncvmf/sections/0-Abs.tex <==
\begin{abstract}
Large language models (LLMs) have shown increasing power on various natural language processing (NLP) tasks.
However, 
tuning these models for downstream tasks usually 
% cause 
needs
exorbitant costs or is unavailable due to commercial considerations.
% Previous works employ black-box tuning, 
% which optimizes task-specific prompts without accessing the gradients and hidden representations, 
% to address this problem.
Recently, 
black-box tuning has been proposed to address this problem by optimizing task-specific prompts without accessing the gradients and hidden representations.
However, 
% past work 
most existing works have
% has 
yet 
% to 
fully exploited the potential of gradient-free optimization under the scenario of few-shot learning.
In this paper, 
we describe BBT-RGB, 
a suite of straightforward and complementary techniques for enhancing the efficiency and performance of black-box optimization. 
Specifically,
our method includes three plug-and-play components:
(1) Two-stage derivative-free optimization strategy that facilitates fast convergence and mitigates overfitting; 
(2) Automatic verbalizer construction with its novel usage under few-shot settings;
(3) Better prompt initialization policy based on instruction search and auto-selected demonstration.
Extensive experiments across various tasks 
% of
on
natural language understanding and inference demonstrate the effectiveness of our method. 
Our codes and data are available at \url{https://github.com/QiushiSun/BBT-RGB}.


\end{abstract}

==> xnjbvwytkznyvkjxpkjxwdqtrytncvmf/sections/1-Intro.tex <==
\section{Introduction}
\label{sec:intro}
Transformer-based Language models~\cite{vaswani2017attention} have achieved remarkable improvements among various NLP tasks~\cite{qiu2020pre, lin2022transformer} in recent years.
These models are mainly first pre-trained on a large-scale unsupervised corpus and then fine-tuned on a specific downstream task.
However, 
this paradigm of {pre-train and fine-tune} face challenges in the era of Large Language Models (LLMs)~\cite[][\emph{inter alia}]{brown2020GPT3, ouyang2022trainingLM, chowdhery2022palm, zhang2022opt, scao2022bloom, touvron2023llama, openai2023gpt4}.
The ever-growing model size leads to a non-stop increase in the cost of tuning, and deploying separate copies of LLMs in real applications becomes exorbitantly expensive.
Though recent research on parameter-efficient tuning~\cite[][\emph{inter alia}]{li2021prefix, lester2021power} alleviates the problem by tuning a small percentage of parameters while keeping the backbone frozen, 
the second problem arises: \textit{most LLMs are released as a service, and users can only access them through Black-Box APIs.} 
% question This implies that the previously mentioned tuning strategies become less viable owing to the unavailability of parameters and gradients, thereby creating a conundrum for subsequent applications.
This implies that the aforementioned tuning strategies become less viable owing to the inaccessibility of parameters and gradients, 
thereby causing a dilemma for downstream applications.
\citet{sun2022bbt} describe this scenario as Language Model-as-a-Service (LMaaS): 
Users are unable to tune the model parameters but can accomplish the tasks of interest by finding appropriate prompts with limited examples. 
Then, Black-Box Tuning (BBT) is proposed as a framework for derivative-free optimization under few-shot settings. 
Recently, BBTv2~\citep{sun2022bbtv2}  has been presented as an improved version that prepends prompts to hidden states of models instead of only injecting prompt tokens in the input layer.
However, 
the potential of black-box optimization is still not fully exploited.
Previous tuning methods are prone to overfit / fall into local optimum under the scenario of few-shot learning. 
This phenomenon is triggered by both the characteristics of the Derivative-free optimization (DFO) algorithm and the unavailability of pre-trained prompts under few-shot settings. 

% \sqs{more details required}
% \sqs{from prompt learning -> verbalizer and instruction ; from opt -> two stage}

In this paper, 
we present BBT-RGB, 
a suite of straightforward, 
complementary, and pluggable techniques that further explore the possibility of black-box tuning. 
We take one step forward in black-box tuning from the following three aspects 
1) Employing a two-stage DFO strategy for the attenuation of overfitting.
2) Utilizing multiple auto-selected verbalizers to exploit the context further.
3) Combining manual prompt with new search approach for task instructions improvement. 

Extensive experiments across various NLP downstream tasks demonstrate the superiority of our method.
Besides,
BBT-RGB can significantly outperform current gradient-based Parameter-Efficient tuning methods~\cite{houlsby2019ParamEff, Zaken2022bitfit, hu2022lora, liu2022ptuning} under the scenario of few-shot learning.
% Moreover, 


Our main contributions can be summarized as follows:
\begin{itemize}[itemsep=6pt,topsep=0pt,parsep=0pt]
    \item We propose a two-stage derivative-free optimization strategy that enables stable convergence of training tunable prompts while effectively mitigating the issue of overfitting.
    \item To further exploit the LLM's output, we propose a verbalizer selection process to derive multiple appropriate candidates. Moreover, 
    instruction with judiciously selected demonstration is adopted for prompt initialization.
    \item 
    % As is shown in Figure~\ref{fig:param-vis}, 
    A wide range of NLP tasks is covered to verify the effectiveness of our approach. 
    By employing our method, 
    optimization\footnote{
    We follow bbtv2~\cite{sun2022bbtv2} to use random projection matrices to transform prompt parameters into low-dimensional subspaces.
} under the derivative-free framework can reach comparative performance to full fine-tuning.
% while preserving much fewer tunable parameters.
    % Additionally, we further discuss the benefits BBT-RGB brings to black-box optimization.
    % reasons why these add-ons function well on different types of tasks.
\end{itemize}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.88\linewidth]{figures/bbt-rgb-BBT-RGB.drawio.pdf}
    \caption{An illustration of BBT-RGB. 
    Given a backbone model with $L$ layers.
    The target is to optimize continuous prompts $z^{l}, l\in [1, L]$.
    We use {\color{BrickRed}{\textbf{R}ed}}, {\color{ForestGreen}{\textbf{G}reen}} and {\color{LakeBlue}{\textbf{B}lue}} to indicate three distinct aspects of our strategy, which inspired the naming of our method. 
    {\color{LakeBlue}{M\textsuperscript{2}} Verbalizers} (Multi-Mixed Verbalizers) further utilize the information provided by the LLMs.
    {\color{ForestGreen}{In\textsuperscript{2}} Initialization} (Instruction learning + In-context learning) improves prompt-based tuning by integrating both instruction and demonstration,
    noted as $p_{l }$.
    And {\color{BrickRed}{Two-Stage DFOs}} exploit the advantages of different optimization methods. \includegraphics[width=.35cm, valign=c]{figures/dfos.png}\ represents the combination of derivative-free optimizers.
    (Best viewed in color.)
    }
    \label{fig:overview}
    \vspace{-0.75em}
\end{figure*}


==> xnjbvwytkznyvkjxpkjxwdqtrytncvmf/sections/2-Prelim.tex <==
\section{Preliminaries}

% In this section, we briefly introduce the basics of LLMs, prompt-based learning, and DFO.

 \subsection{Large Language Models and APIs}

Large language models (LLMs)~\cite{devlin2018bert, liu2019roberta, brown2020GPT3} have revolutionized the NLP landscape in the past few years. 
Given some examples of tasks as input, 
LLMs can be ``prompted'' to conduct a wide range of NLP tasks.
These huge models are usually released as a service~\cite{brown2020GPT3, chen2021evaluating, ouyang2022trainingLM}, which allows users to interact with the models deployed on the cloud servers through APIs.
Unlike some popular open-source LMs~\cite{devlin2018bert, liu2019roberta} that can be directly utilized by researchers, 
access to the parameters and gradients of LLMs is restricted due to commercial, ethical, and security concerns.

\subsection{Prompt-based Learning}

Prompt-based learning~\cite{liu2021promptsurvey} transforms an NLP downstream task into a masked language modeling (MLM) task and narrows the discrepancy between pre-training and fine-tuning.
Based on the prompt format, 
prompt-based learning can be categorized into discrete prompts and continuous prompts.
Discrete prompts can be designed manually~\citep{brown2020GPT3, schick2020automatically} or generated automatically~\cite{gao2021making}.
Continuous prompts are designed as a sequence of vectors~\cite{qin2021learning, lester2021power} that are usually prepended to the input and optimized by gradients.
Recently,~\citet{sun2022bbt} propose BBT for optimizing prompts under gradient-free settings, as is shown in section~\ref{sec:bbt}.
We mainly focus on the optimization of continuous prompts under the black-box settings in this paper.

% , for more details, please refer to Appendix~\ref{sec:rw-bb}.

% optimize the prepended continuous prompt tokens.

\subsection{Derivative-free Optimization}

Derivative-free optimization (DFO) algorithms are capable of solving complex problems without the back-propagation process. 
DFO generally employs a sampling-and-updating framework~\cite{rios2013DFOreview, wierstra2014nes, qian2016dfo} to improve the solution iteratively.
For instance, 
Covariance Matrix Adaptation Evolution Strategy~\cite{hansen2001cma, hansen2003reducing}, namely CMA-ES, 
is a widely adopted evolutionary algorithm for non-linear non-convex continuous optimization.
At each iteration, 
the algorithm samples new potential solutions from a parameterized distribution model (\textit{e.g.}, multivariate normal distribution).
Besides,
we have COBYLA algorithm (Constrained Optimization BY Linear Approximation)~\cite{powell1994direct, powell1998direct} that builds a linear approximation model of the objective function and constraints within a trust region, 
iteratively updating the model based on the progress made in minimizing the objective function.


% Powell algorithm~\cite{powell1964efficient} and COBYLA algorithm (Constrained Optimization BY Linear Approximation)~\cite{powell1994direct, powell1998direct} are also classic search-based DFO algorithms.


==> xnjbvwytkznyvkjxpkjxwdqtrytncvmf/sections/3-Model.tex <==
\section{BBT-RGB}
As is shown in Figure~\ref{fig:overview},
we introduce our method: BBT-RGB, 
which contains three orthogonal optimization perspectives of derivative-free learning\footnote{The backgrounds and formal definition of derivative-free learning methods are given in section~\ref{sec:bbt}.}.


\subsection{Two-Stage DFOs}
Previous works of black-box tuning mainly use CMA-ES to optimize the intrinsic dimensionality~\cite{aghajanyan2021intrinsic} of LLMs.
Nonetheless,
in the early training stage, 
the evolutionary algorithm (EA) exhibits a considerably faster convergence rate compared to the search-based algorithm (SA),
which potentially causes fast overfitting.
Then, the following steps would be futile.
Thus, we design a novel two-stage DFO algorithm\footnote{Due to space limitations, we put the detailed algorithm in Appendix~\ref{sec:two-stage-detailed}.
Algorithm~\ref{alg:two-stage} stands for a simplified version.} for black-box tuning, 
as is shown in algorithm~\ref{alg:two-stage}. 

\begin{algorithm}[t]
	\caption{Two-Stage DFOs}
	\label{alg:two-stage}
	\begin{algorithmic}[1]
		\Require \
		 popsize:$\lambda$, intrinsic dimension:$d$
            \Require \
          budget1:$b1$, budget2:$b2$, backbone:$f_{model}$
		\Ensure \
		hidden variable: $z$
		\Function{Two-Stage DFO}{}   
            \Repeat
            \For{each hidden layer}
            \State Update $z$ by Evolutionary DFO
            \EndFor
            \Until{ $b1$ times $f_{model}$ call}
            \For{each hidden layer}
            \Repeat
            \State Update $z$ by Search-based DFO
            \Until{ $b2//d$ times $f_{model}$ call}
            \EndFor
            % \EndFor
	    \EndFunction
	\end{algorithmic}
\end{algorithm}

We leverage the advantages of two different kinds of DFOs respectively.
In stage \uppercase\expandafter{\romannumeral1}, we use EA to perform coarse-grained population-level optimization, which has a specific budget (Number of API Calls) to move toward the target swiftly.
And the SA will use the remaining budgets in stage \uppercase\expandafter{\romannumeral2} for approximating the solution by dimension-level fine-grained search.

\input{tables/main-result}

\subsection{M\textsuperscript{2} Verbalizers}

Most prior works employ a single verbalizer for gradient-free optimization, which cannot make full use of the information, \textit{i.e.}, logits returned by the black box model.
To address this problem, 
we propose \textbf{M}ulti-\textbf{M}ixed verbalizers, 
which are constructed through the following methods: 
1) manual verbalizer selection\footnote{Specifically, we use synonyms in practice.}. 
2) search-based verbalizer construction based on word importance estimation by TF-IDF.
3) auto verbalizer generation based on neural nets~\cite{gao2021making}.
After verbalizers are selected by the aforementioned approaches, the confidence of each category is represented by the average prediction probability of multiple verbalizers.
Compared with the previous approach, 
M\textsuperscript{2} verbalizers make one step forward to exploit the information provided by the black-box model.
Additionally, this approach can prevent the negative impact on model performance caused by a single unsuitable label word.

\subsection{In\textsuperscript{2} Initialization}
An appropriate initialization has proven to play an essential role in effective prompt-based tuning~\cite{an2022input, prasad2022GrIPS}.
Inspired by previous efforts, we propose a model-agnostic strategy named as In\textsuperscript{2} initialization.
The first component of our approach is a task-specific manual \textbf{In}struction.
For the second part, we iterate through the training set and take each sample as a demonstration~\cite{sewon2022rethinking},
which is assessed on the validation set together with the pre-selected instruction. 
After that, the sample with the best performance is selected for \textbf{In}-context learning.



==> xnjbvwytkznyvkjxpkjxwdqtrytncvmf/sections/4-Exp.tex <==
\section{Experiments}

\subsection{Experimental Settings}
\label{exp:settting}

\paragraph{Backbone}
We use RoBERTa-Large~\cite{liu2019roberta} as backbone throughout the experiments.

% \footnote{\url{https://huggingface.co/roberta-large}}


\paragraph{Datasets}
To evaluate our proposed methods, 
we choose a series of tasks from the GLUE benchmark~\cite{wang2018glue}.
Specifically, we employ SST-2~\cite{socher2013sst} and Yelp~\cite{zhang2015char} for sentiment analysis, AGNews and DBPedia~\cite{zhang2015char} for topic classification, SNLI~\cite{bowman2015snli} and RTE~\cite{dagan2005the} for natural language inference, and MRPC~\cite{dolan2005mrpc} for semantic paraphrasing.

\paragraph{Methods and Hyperparameters} For all the experiments we covered, 
the components of BBT-RGB we employed and hyperparameters are showcased in Table~\ref{table:rgb-settings} and Table~\ref{table:hparams}.
The details of experimental settings are listed in secion~\ref{sec:exp-details}.
% The details of ablation studies are listed in section~\ref{sec:ablation}.

% \sqs{under construction}

\subsection{Main Results}

As is demonstrated in table~\ref{tab:main}, 
we compare BBT-RGB with both gradient-based and gradient-free tuning methods\footnote{We employ the results reported by~\citet{sun2022bbtv2} for comparison.}. 
We observed different levels of improvement on various NLP tasks.

\paragraph{Sentiment Analysis}
On both the SST-2 and Yelp datasets,
our method surpasses all prior white-box methods, 
consistently demonstrating superior performance compared to the established baselines.

\paragraph{Topic Classification}
Compared with the previous gradient-free method, BBT-RGB has a significant advancement in the evaluation based on DBPedia and AGNews but still needs to catch up to full model tuning.
We hold the view that this is caused by a relatively large number of classes (categories), and it is difficult for the model to learn enough knowledge under few-shot settings.

\paragraph{Entailment and Inference}
BBT-RGB benefits entailment and natural language inference tasks significantly; both experiments on SNLI and MRPC indicate surpassing full fine-tuning performance. 
In addition, we can observe a leap in the accuracy of RTE compared with previous baselines.


\subsection{Ablation Studies and Analysis}
\label{sec:ablations}

\paragraph{Ablation Studies.}
We conduct ablation studies to verify the effectiveness of the three proposed techniques that formed the core of this paper,
as demonstrated in Table~\ref{tab:ablations}. 
Overall, each component of BBT-RGB demonstrates gains across various tasks.

\input{tables/ablations}

To balance computational resource constraints and fairness,
we select one task each from Sentiment Analysis, Topic Classification, and Entailment \& Inference. 
Then we carry out ablation studies on each module comprising BBT-RGB (with \texttt{random seed = 42}).


\paragraph{Performance and Stability Comparison.}

Figure~\ref{fig:param-vis} illustrates a comparative analysis of BBT-RGB against other gradient-based and gradient-free methods in terms of performance, parameter tuning requirements, and stability. 

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.38]{figures/vis/bbt-rgb-params.pdf}
    \caption{Comparing BBT-RGB with other tuning methods on average performance over seven tasks described in section~\ref{exp:settting}.
    The size of the circle is proportional to the standard deviation.}
    \label{fig:param-vis}
\end{figure}

It is evident that while maintaining optimal performance, BBT-RGB incurs minimal computational overhead. Moreover, the standard deviation indicates BBT-RGB's superior stability compared to these methods, attributable to In\textsuperscript{2} Initialization enhancing the stability of few-shot learning.

% Case studies for individual tasks can be found in section~\ref{appendix:case}.
Case studies pertaining to the optimization process can be found in section~\ref{appendix:case}. 


==> xnjbvwytkznyvkjxpkjxwdqtrytncvmf/sections/5-Conc.tex <==
\section{Conclusion}
This paper proposes BBT-RGB, 
a set of simple but effective techniques to drive more powerful derivative-free prompt-based learning.
% enhance black-box tuning.
% Our method 
% when the parameters and gradients of the model are invisible.
We make improvements from three independent aspects: 
(1) Two-stage derivative-free optimization algorithms for attenuating overfitting; 
(2) Versatile verbalizer construction with a robust selection process; 
(3) Using Instruction learning and demonstrations to exploit in-context information.
All the modules are ``plug-and-play'', 
and empirical studies across a series of tasks verify the effectiveness of our method.

==> xnjbvwytkznyvkjxpkjxwdqtrytncvmf/sections/6-Lim.tex <==
\section*{Limitations and Ethical Consideration}

\paragraph{Limitations.}
Our limitations are threefold:
\begin{itemize}
    \item Following previous works~\citep{sun2022bbt, sun2022bbtv2},
our proposed method lays much emphasis on the optimization of continuous prompts.
It can be applied to a majority of open-source Large Language Models (LLMs), but for some commercial models that do not provide loss, logits, or perplexity, the optimization is constrained to remain in the discrete form at the initial layer of the model.
    \item Since the algorithm is unable to achieve linear convergence,
some of the tasks require more API calls,
which may lead to extra costs when running on commercial models.
    \item Given that In\textsuperscript{2}Init and M\textsuperscript{2}Verb involve the search for verbalizers and demonstrations, our method takes a longer execution time compared to BBTv2, requiring approximately 25\% additional runtime.
\end{itemize}

\paragraph*{Ethical Considerations.}
Our method: BBT-RGB, aims to exploit the potential of black-box tuning further, and the contribution in this paper is fully methodological. 
Therefore, this contribution has no direct negative social or ethical impacts.
Moreover, 
given that our approach requires significantly less computational resources compared to full-fine tuning, 
it is poised to contribute positively to the sustainable development of the community.


\section*{Acknowledgment}
This work is supported by Shanghai ``Science and Technology Innovation Action Plan'' Project (No.23511100700).
Our method is also derived from a prize-winning solution of the \textit{First International Algorithm Case Competition: PLM Tuning Track, Guangdong-Hong Kong-Macao Greater Bay Area}.
Finally, 
we thank our anonymous reviewers for their insightful comments and suggestions.


==> xnjbvwytkznyvkjxpkjxwdqtrytncvmf/sections/7-Apdx.tex <==

\input{sections/8-bbt.tex}




% \section{Ablation Studies}
% \label{sec:ablation}

% We conduct ablation studies to verify the effectiveness of the three proposed techniques that formed the core of this paper.

% \input{tables/ablations}


\section{Detailed Two-Stage DFOs Algorithm}
\label{sec:two-stage-detailed}

Algorithm~\ref{alg:two-stage-detailed} is the full version of the Two-Stage DFOs we used in this paper. For the Evolutionary algorithm and the search-based algorithm, we select CMA-ES and COBYLA, respectively.

\input{algs/two-stage}

\section{Case Studies}
\label{appendix:case}

% \subsection{Analysis}

We select two cases\footnote{We choose CMA-ES (8,000 budgets) and COBYLA (12,000 budgets) for the two-stage DFOs in this illustration.} 
to analyze the effectiveness of two-stage DFOs on Yelp dataset. 
In Figure~\ref{fig:2stage-comp}, 
the training loss (orange curve) converges to zero for both methods.
While the oscillation of validation loss observed in pure CMA-ES case is mainly attributed to the nature of the adaptive algorithm.

\begin{figure}[ht]
    \centering
    \subfigure[CMA-ES]{
	\includegraphics[width=0.231\textwidth]{figures/vis/Yelp-2w-no-2stage.pdf}
	\label{pic1:yelp-no2stage}
    }
    \subfigure[Two-Stage DFOs]{
	\includegraphics[width=0.22\textwidth]{figures/vis/Yelp-8k-1w2-cma-cobyla.pdf}
	\label{pic1:yelp-2stage}
    }
    \caption{Comparison of original CMA-ES and Two-stage DFOs on Yelp dataset.}
    \label{fig:2stage-comp}
\end{figure}

In stage II of our proposed two-stage DFOs method, 
a relatively gentle decrease in validation loss can be observed,
demonstrating that dimension-level updates by COBYLA make the overall learning process smoother, which helps us curb the problem of fast overfitting.
% Another case can be found in section~\ref{appendix:case}.
% Our method largely curbs the problem that training loss decreases while validation loss (blue curve) increases and oscillates.

Figure~\ref{fig:sst2-2stage} is another analysis of SST-2 dataset.
By employing the Two-stage DFOs (Blue line),
there is a notable improvement in the final optimization result.

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.16]{figures/vis/SST-2-two-stage.pdf}
    \caption{An illustration of Two-Stage DFOs on SST-2}
    \label{fig:sst2-2stage}
\end{figure}

\section{Experimental Details}
\label{sec:exp-details}

\subsection{Implementation}
Most of our experiments are conducted with a single NVIDIA RTX 3090 GPU. 
Due to the memory requirements, 
experiments on MRPC and DBPedia datasets are conducted with NVIDIA V100 GPUs.
% \footnote{Due to the memory requirements, experiments on MRPC and DBPedia datasets are conducted with NVIDIA V100 GPUs.}

\subsection{BBT-RGB Settings}
\label{sec:rgb-setting}

The details of using BBT-RGB across seven NLP tasks are listed in Table~\ref{table:rgb-settings}.
For each task, 
we report the average performance and standard deviation across three random seeds (42, 50, 66).

\begin{table*}[t]
\begin{center}
		\begin{tabular}{lccccccc}
			\toprule
			& SST-2 & Yelp & AGNews & DBPedia & SNLI & RTE &MRPC \\
			\midrule
                Two-Stage DFO & \color{ForestGreen}{\Checkmark} & \color{ForestGreen}{\Checkmark} & \color{ForestGreen}{\Checkmark} &
                \color{ForestGreen}{\Checkmark} &\color{ForestGreen}{\Checkmark} & \color{ForestGreen}{\Checkmark} & \color{BrickRed}{\XSolidBrush} \\
			M\textsuperscript{2} Verbalizers & \color{BrickRed}{\XSolidBrush} & \color{ForestGreen}{\Checkmark} & \color{BrickRed}{\XSolidBrush} & \color{ForestGreen}{\Checkmark} & \color{BrickRed}{\XSolidBrush} & \color{ForestGreen}{\Checkmark} &
			\color{ForestGreen}{\Checkmark}\\
			In\textsuperscript{2} Initialization &  \color{ForestGreen}{\Checkmark} & \color{ForestGreen}{\Checkmark} & \color{ForestGreen}{\Checkmark} & \color{ForestGreen}{\Checkmark} & \color{ForestGreen}{\Checkmark} &
			\color{ForestGreen}{\Checkmark} & \color{BrickRed}{\XSolidBrush} \\
			\bottomrule
		\end{tabular}
		\caption{The details of employing BBT-RGB, {\color{ForestGreen}{\Checkmark}} refers to use the given technique on this task, and {\color{BrickRed}{\XSolidBrush}} vice versa}
		\label{table:rgb-settings}
\end{center}
\end{table*}


\subsection{Hyperparameters Settings}
\label{sec:hyper-params}

The experimental settings in our paper are listed in Table~\ref{table:hparams}. Sigma1 and Sigma2 are the hyperparameters for CMA-ES. Alpha refers to a constant scalar for stretching the distribution of random projection matrices, as is shown in equation~\ref{eq:sigma}.

\begin{equation}
    \sigma_A = \frac{\alpha\hat{\sigma}}{\sqrt{d}\sigma_z},
    \label{eq:sigma}
\end{equation}

$\hat{\sigma}$ is the standard deviation of word embeddings from RoBERTa-Large, and $\sigma_z$ is the standard deviation of the normal distribution maintained by the CMA-ES algorithm.
The random projection matrices are frozen during the whole optimization process.

\input{tables/hparams}

\subsection{Templates and Verbalizers}

The templates and verbalizers we employed are listed in Table~\ref{tab:template-verb} and Table~\ref{tab:m2verbalizer} respectively.

\input{tables/template-verb}

\input{tables/m2verb}

% The details of using BBT-RGB and hyperparameter settings are listed in table~\ref{table:rgb-settings} and section~\ref{sec:hyper-params} respectively.







==> xnjbvwytkznyvkjxpkjxwdqtrytncvmf/sections/8-bbt.tex <==
\section{Derivative-Free Prompt Tuning}
\label{sec:bbt}
% We provide a formal definition of BBT and discuss recent research progress in the field in this section. 
% \subsection{Background}
Given a batch of samples $(X, Y)$ converted with prompt templates and label words,
the original derivative-free prompt learning, as introduced by~\citet{sun2022bbtv2} first use a set of prompt embeddings $p$ to concatenate the input tokens, 
creating the prompted input for LLMs with frozen backbones.
The prompt $p = p_0 + p_\theta$ consists of the initial prompt $p_0 \in \mathbb{R}^D$, which is manually/randomly selected and a tunable prompt $p_\theta \in \mathbb{R}^{D}$ that is progressively optimized through a DFO algorithm like CMA-ES~\citep{hansen2003reducing}. 
DFOs suffer slow convergence on high-dimensional problems,
but fortunately, \citet{aghajanyan2021intrinsic} discover that PLMs exhibit low-dimensional reparameterization that is as effective for fine-tuning as the full parameter space. 
This finding indicates that the search space of $p_\theta$ can be condensed into an intrinsic dimensionality ${z} \in \mathbb{R}^d ~(d \ll D)$ by using a (frozen) random projection matrix $\Pi\in\mathbb{R}^{D \times d}$, 
such that $p_\theta = \Pi \cdot {z} $ will
significantly decrease the cost of optimization.
Subsequently, the task-specific inference of model $f$ through API Call is performed to determine the fitness of candidate prompts using an objective function $\mathcal{L}(f([P;X]), Y)$, where $\mathcal{L}$ is a loss function such as cross-entropy.
Finally, 
the DFO algorithm iteratively refines the prompt for seeking ${p^{*}} = \arg\min_{p} \mathcal{L} (f([P;X]), Y)$.

% \label{sec:def}
% \subsection{Black-Box Optimization Approaches}
% \label{sec:rw-bb}
% \sqs{waiting for modification} 

In the era of large language models, 
black-box optimization is a promising research target that can drive models for few-shot learning without access to gradients. 
\citet{sun2022bbt} first propose BBT that focuses on optimizing continuous prompt by only accessing inference APIs 
and then present BBTv2~\cite{sun2022bbtv2} as an improved version.
While some recent works
%, there are also some studies that 
focus on optimizing discrete prompts concurrent with our work.
\citet{Diao2022bbp} present black-box discrete prompt learning with gradient estimation as their key feature.
\citet{hou2022promptboosting} first use gradient-free methods to sample sub-optimal discrete prompts and then ensemble them by boosting algorithm. And \citet{chai2022clip} acquire informative feedback to enhance derivative-free optimization through using frozen subnetworks as critics.
Recently, \citet{han2023gdfo} ingeniously leverage knowledge distillation to combine gradient descent and gradient-free optimization.

==> xnjbvwytkznyvkjxpkjxwdqtrytncvmf/tables/ablations.tex <==
\begin{table}[ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{SST-2} & \textbf{AG's News} & \textbf{RTE} \\ 
% \textbf{Method} & \textbf{SST-2(1821)} & \textbf{AG's News(7600)} & \textbf{RTE3000} \\ 
\midrule
\textbf{BBT-RGB} & 91.00     & 85.59        & 61.80      \\
\midrule
~w/o. M\textsuperscript{2}Verb    & 91.00      & 85.59      & 61.33      \\
~w/o. Two-Stage     & 90.39      & 85.57        & 61.17  \\ 
~w/o. In\textsuperscript{2}Init     & 90.77      & 84.31        & 60.17  \\
\midrule
~w/o. Two-Stage \& M\textsuperscript{2}Verb   & 90.83      & 85.56        & 59.77 \\ 
~w/o. Two-Stage \& In\textsuperscript{2}Init   & 90.28      & 83.79        & 59.30  \\ 
~w/o. In\textsuperscript{2}Init \& M\textsuperscript{2}Verb   & 90.66      & 83.75        & 59.47  \\ 

\bottomrule
\end{tabular}
}
\caption{Ablation studies of BBT-RGB on SST-2, AG's News, and RTE}
\label{tab:ablations}
\end{table}

==> xnjbvwytkznyvkjxpkjxwdqtrytncvmf/tables/hparams.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{0.8\textwidth}{!}{
		\begin{tabular}{lccccc}
			\toprule
			Task & Budget1 (CMA-ES) & Budget2 (COBYLA) & Alpha & Sigma1 & Sigma2 \\
			\midrule
            SST-2 & 7,000 & 6,000 & 0.5 & 0.7 & 0.7  \\
            Yelp & 8,000 & 6,000 & 0.9 & 0.4 & 0.2  \\
            \cdashline{1-6}
            AGNews & 8,000 & 6,000 & 0.1 & 0.6 & 0.2  \\
            DBPedia & 8,000 & 6,000 & 0.3 & 0.2 & 0.2 \\
            \cdashline{1-6}
            SNLI & 8,000 & 6,000 & 0.5 & 0.45 & 0.2  \\
            RTE & 8,000 & 6,000 & 0.5 & 1 & 0.2  \\
            MRPC & 8,000 & 0 & 0.3 & 0.3 & 0.2  \\
			\bottomrule
		\end{tabular}
		}
		\caption{Hyperparameter Settings for BBT-RGB in different tasks.}
		\label{table:hparams}
\end{center}
\end{table*}

==> xnjbvwytkznyvkjxpkjxwdqtrytncvmf/tables/m2verb.tex <==
\begin{table*}[t]
\centering
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{ll}
\toprule
\textbf{Dataset} & \textbf{M\textsuperscript{2} Verbalizers} \\ 
\midrule
\multirow{2}{*}{SST-2}  & \textbf{Positive}: exciting, all, indeed, $\cdots$   \\
& \textbf{Negative}: ridiculous, worse, stupid, $\cdots$ \\
\cdashline{1-2}
\multirow{2}{*}{Yelp P.} & \textbf{Positive}: addictive, sensational, classic, $\cdots$ \\
& \textbf{Negative}: boring, worse, ugly, $\cdots$  \\
\cdashline{1-2}
\multirow{4}{*}{AG's News} & \textbf{World}: South, China, Africa, $\cdots$ \\
& \textbf{Sports}: Athletics, SPORTS, Sporting, $\cdots$ \\
& \textbf{Business}: Banking, Manufacturing, Trade, $\cdots$ \\
& \textbf{Tech}: Digital, Internet, Tech, $\cdots$ \\
\cdashline{1-2}
\multirow{14}{*}{DBPedia} & \textbf{Company}: Business, Products, $\cdots$ \\
& \textbf{Educational/Institution}: Education, Schools, $\cdots$ \\
& \textbf{Artist}: Artists, $\cdots$ \\
& \textbf{Athlete}: Profile, $\cdots$ \\
& \textbf{Office Holder}: Politics, $\cdots$ \\
& \textbf{Mean Of Transportation}: Vehicles, $\cdots$ \\
& \textbf{Building}: Architecture, $\cdots$ \\
& \textbf{Natural Place}: Lakes, $\cdots$ \\
& \textbf{Village}: Rural, $\cdots$ \\
& \textbf{Animal}: Animals, Birds, $\cdots$ \\
& \textbf{Plant}: Plants, plants, Flowers, $\cdots$ \\
& \textbf{Album}: Album, Records, $\cdots$ \\
& \textbf{Film}: Movies, Films, $\cdots$ \\
& \textbf{Written Work}: Books, Fiction, $\cdots$ \\
\cdashline{1-2}
\multirow{2}{*}{MRPC} & \textbf{Equivalent}: Finally, Notably, Next, $\cdots$ \\
& \textbf{Not Equivalent}: Instead, Although, That, $\cdots$ \\
\cdashline{1-2}
\multirow{2}{*}{RTE} &  \textbf{Yes}: Indeed, So, Wordwide, $\cdots$ \\
& \textbf{No}: Also, Now, meanwhile, $\cdots$ \\
\cdashline{1-2}
\multirow{3}{*}{SNLI} & \textbf{Yes}: Whatever, YES, Regardless, $\cdots$ \\
& \textbf{Maybe}: Imagine, Usually, Typically, $\cdots$ \\
& \textbf{No}: Besides, Unfortunately, Surprisingly, $\cdots$ \\
\bottomrule
\end{tabular}
}
\caption{Examples of the M\textsuperscript{2} Verbalizers used in practice.}
\label{tab:m2verbalizer}
\end{table*}

==> xnjbvwytkznyvkjxpkjxwdqtrytncvmf/tables/main-result.tex <==
\begin{table*}[t]
\centering
\label{tab:main_results}
\resizebox{1.01\linewidth}{!}{
\begin{tabular}{lcccccccr}
\toprule
\multirow{2}{*}{\textbf{Method}} & \textbf{SST-2} & \textbf{Yelp P.} & \textbf{AG's News} & \textbf{DBPedia} & \textbf{MRPC} & \textbf{SNLI} & \textbf{RTE} & \multirow{2}{*}{\textbf{Avg.}} \\
& acc  & acc  & acc & acc & F1 & acc & acc & \\ 
\midrule
\multicolumn{9}{c}{\textit{Gradient-Based Methods}} \\ 
\midrule
Model Fine-Tuning & {85.39} \small{$\pm$2.84} & {91.82} \small{$\pm$0.79} & 86.36 \small{$\pm$1.85} & {97.98} \small{$\pm$0.14} & {\textbf{77.35}} \small{$\pm$5.70} & 54.64 \small{$\pm$5.29} & {\textbf{58.60}} \small{$\pm$6.21} & {78.88}\\
Prompt Tuning~\cite{lester2021power} & 68.23 \small{$\pm$3.78} & 61.02 \small{$\pm$6.65} & 84.81 \small{$\pm$0.66} & 87.75 \small{$\pm$1.48} & 51.61 \small{$\pm$8.67} & 36.13 \small{$\pm$1.51} & {54.69} \small{$\pm$3.79} & 63.46 \\
P-Tuning v2~\cite{liu2022ptuning} & 64.33 \small{$\pm$3.05} & {\textbf{92.63}} \small{$\pm$1.39} &83.46 \small{$\pm$1.01} &97.05 \small{$\pm$0.41} &68.14 \small{$\pm$3.89} &36.89 \small{$\pm$0.79} &50.78 \small{$\pm$2.28} & 70.47 \\ 
Adapter~\cite{houlsby2019ParamEff} & 83.91 \small{$\pm$2.90} & 90.99 \small{$\pm$2.86}  & 86.01 \small{$\pm$2.18} & {\textbf{97.99}} \small{$\pm$0.07} & 69.20 \small{$\pm$3.58} & {57.46} \small{$\pm$6.63} & 48.62 \small{$\pm$4.74} & 76.31 \\ 
LoRA~\cite{hu2022lora} & {\textbf{88.49}} \small{$\pm$2.90} & 90.21 \small{$\pm$4.00} & {\textbf{87.09}} \small{$\pm$0.85} & 97.86 \small{$\pm$0.17} & {72.14} \small{$\pm$2.23} & {\textbf{61.03}} \small{$\pm$8.55} & 49.22 \small{$\pm$5.12} & {78.01} \\
BitFit~\cite{Zaken2022bitfit} & 81.19 \small{$\pm$6.08} & 88.63 \small{$\pm$6.69} & {86.83} \small{$\pm$0.62} & 94.42 \small{$\pm$0.94} & 66.26 \small{$\pm$6.81} & 53.42 \small{$\pm$10.63} & 52.59 \small{$\pm$5.31} & 74.76 \\  
\midrule
\multicolumn{9}{c}{\textit{Gradient-Free Methods}} \\ 
\midrule
Manual Prompt & 79.82 & 89.65 & 76.96 & 41.33 & 67.40 & 31.11 & 51.62 & 62.56 \\
In-Context Learning~\cite{brown2020GPT3} & 79.79 \small{$\pm$3.06} & 85.38 \small{$\pm$3.92} & 62.21 \small{$\pm$13.46} & 34.83 \small{$\pm$7.59} & 45.81 \small{$\pm$6.67} & {47.11} \small{$\pm$0.63} & {60.36} \small{$\pm$1.56} & 59.36\\
\cdashline{1-9}
BBT~\cite{sun2022bbt} & {89.56} \small{$\pm$0.25} & {91.50} \small{$\pm$0.16} & {81.51} \small{$\pm$0.79} & 79.99 \small{$\pm$2.95} & 61.56 \small{$\pm$4.34} &  46.58 \small{$\pm$1.33}  & 52.59 \small{$\pm$2.21} & {71.90} \\
BBTv2~\cite{sun2022bbtv2} & 90.33 \small{$\pm$1.73} & 92.86 \small{$\pm$0.62} & {85.28} \small{$\pm$0.49} & 93.64 \small{$\pm$0.68} & 77.01 \small{$\pm$4.73} & 57.27 \small{$\pm$2.27} & {56.68} \small{$\pm$3.32} & 79.01 \\ 
\textbf{BBT-RGB (ours)} & \textbf{92.89} \small{$\pm$0.26} & \textbf{94.20} \small{$\pm$0.48} &  \textbf{85.60} \small{$\pm$0.41} &\textbf{94.41} \small{$\pm$0.73}  & \textbf{79.49} \small{$\pm$1.84} & \textbf{60.71} \small{$\pm$0.66}  & \textbf{61.82} \small{$\pm$1.20} & \textbf{81.30} \\
\bottomrule
\end{tabular}
}
\caption{Overall comparison between BBT-RGB and other methods~(both gradient-based and gradient-free). All of the results are obtained with the RoBERTa-Large~\cite{liu2019roberta} backbone in 16-shot (per class) setting.
The performance of the hitherto best technique combinations is reported in this table, 
as illustrated in Table~\ref{table:rgb-settings}. 
For each distinct combination, 
we demonstrate the ablation stduies in section~\ref{sec:ablations}.
}
\label{tab:main}
\vspace{-1em}
\end{table*}
